Reinforcement Learning-based Fast Charging Control Strategy for Li-ion Batteries

One of the most crucial challenges faced by the Li-ion battery community concerns the search for the minimum time charging without irreversibly damaging the cells. This can fall into solving large-scale nonlinear optimal control problems according to a battery model. Within this context, several model-based techniques have been proposed in the literature.However, the effectiveness of such strategies is significantly limited by model complexity and uncertainty. Additionally, it is difficult to track parameters related to aging and re-tune the model-based control policy. With the aim of overcoming these limitations, in this paper we propose a fast-charging strategy subject to safety constraints which relies on a model-free reinforcement learning framework. In particular, we focus on the policy gradient-based actor-critic algorithm, i.e., deep deterministic policy gradient (DDPG), in order to deal with continuous sets of actions and sets. The validity of the proposal is assessed in simulation when a reduced electrochemical model is considered as the real plant. Finally, the online adaptability of the proposed strategy in response to variations of the environment parameters is highlighted with consideration of state reduction.

==> OptimalCharging.tex <==
\section{Battery Charging Problem}
\label{sec:battchg}

In this section, we introduce the battery charging control problem. In the battery controls literature, researchers have considered the following optimal control problem formulations for battery charging.


% In each formulation, both the ECM and SPMeT models are used for the dynamics. Since the optimal control problems are solved in discrete-time, each model must be discretized in time. In the battery controls literature, researchers have considered the following optimal control problem formulations for battery charging.

%%%
% \subsection{SOC Reference Tracking}
% The SOC reference tracking problem is formulated as:
% \begin{align}
%     \min_{I(t)} & \sum_{t=0}^{t_{f}} \left[ \text{SOC}(t) - \text{SOC}^{\text{r}}(t)\right]^{2} \label{eqn:CtrlProb}\\
%     \text{subject to} & \nonumber \\
%     & \text{Battery model} \nonumber \\
%     & \text{Initial and final conditions} \nonumber \\
%     & \text{Input constraints} \nonumber \\
%     & \text{State constraints} \nonumber 
% \end{align}
% where $\text{SOC}(t)$ is the current SoC at time step $t$, $\text{SOC}^{\text{r}}(t)$ is the reference SoC, and $W$ is a weight. This formulation falls within the class of state reference tracking problems. For battery charging, one might select the reference to be a constant high value of SOC, e.g. $\text{SOC}^{\text{r}}(t) \equiv 0.8 \ \forall \ t \in [0,t_f]$. The authors in \cite{zou2018electrochemical, liu2017extended} have investigated this type of charging problem for health-aware fast charging and computational cost reduction. The authors in \cite{aaron2020nn} proposed a data-driven receding horizon control approach to solve such SOC reference tracking problem.

%%%
\subsection{Minimum time charging}
The minimum time charging problem is formulated as:
\begin{align}
    \min_{I(t),t_f} & \sum_{t=0}^{t_{f}} 1 \label{eqn:Obj_MinTime} \\ 
    \text{subject to} & \nonumber \\
    & \text{equations \eqref{eqn:} \nonumber\\
    & \text{Initial and final conditions} \nonumber \\
    & \text{Input constraints} \nonumber \\
    & \text{State constraints} \nonumber
\end{align}
This is a free-time problem, whose objective is to solve the battery charging problem in minimum time given a battery model and operating constraints. Several publications use this formulation, including \cite{klein2011optimal, perez2017optimal, perez2017optimalJES}. This fast charging problem can be expanded in other forms by modifying the cost function in \eqref{eqn:Obj_MinTime} as maximize the charge throughput over specified time horizon. Work related to this formulation includes \cite{suthar2014optimal, suthar2014optimalJES}. On the other hand, authors in \cite{zou2018electrochemical, liu2017extended, aaron2020nn} consider SOC reference tracking problem where the cost function \eqref{eqn:Obj_MinTime} is defined as squared difference between the current SOC at time step $t$ and the target SOC. This formulation falls within the class of state reference tracking problems.


% %%%
% \subsection{Max charge throughput}
% The maximum charge throughput problem is formulated as:
% \begin{align}
%     \max_{I(t)} & \sum_{t=0}^{t_{f}} I(t) \\
%     \text{subject to} & \nonumber \\
%     & \text{Battery model} \nonumber \\
%     & \text{Initial and final conditions} \nonumber \\
%     & \text{Input constraints} \nonumber \\
%     & \text{State constraints} \nonumber
% \end{align}
% This is a fixed-time charging problem, whose objective is to maximize the charge throughput over a specified time horizon. 




